COSMOS: Coordination of High-Level Synthesis and Memory Optimization for Hardware Accelerators

Hardware accelerators are key to the efficiency and performance of system-on-chip (SoC) architectures. With high-level synthesis (HLS), designers can easily obtain several performance-cost trade-off implementations for each component of a complex hardware accelerator. However, navigating this design space in search of the Pareto-optimal implementations at the system level is a hard optimization task. We present COSMOS, an automatic methodology for the design-space exploration (DSE) of complex accelerators, that coordinates both HLS and memory optimization tools in a compositional way. First, thanks to the co-design of datapath and memory, COSMOS produces a large set of Pareto-optimal implementations for each component of the accelerator. Then, COSMOS leverages compositional design techniques to quickly converge to the desired trade-off point between cost and performance at the system level. When applied to the system-level design (SLD) of an accelerator for wide-area motion imagery (WAMI), COSMOS explores the design space as completely as an exhaustive search, but it reduces the number of invocations to the HLS tool by up to 14.6x.

==> Makefile <==
# Makefile

.PHONY: all clean data

# .tex file
PAPER = paper

# .bib file
REFS = references.bib

# Dependencies

# .tex files
TEX_DEPS = $(wildcard $(PAPER).tex) \
           $(wildcard sections/*.tex)

# .pdf files
FIG_DEPS = $(wildcard figures/pdf/*.pdf)

# Rules

all: $(PAPER).pdf

$(PAPER).pdf: acmart.cls $(TEX_DEPS) $(FIG_DEPS) $(REFS)
	pdflatex $(PAPER)
	@if test -f $(PAPER).aux &&  test `grep citation $(PAPER).aux | wc -l` -ge 1; then bibtex $(PAPER); fi
	pdflatex $(PAPER)
	pdflatex $(PAPER)

%.cls:   %.ins %.dtx
	pdflatex $<

clean:
	rm -f *.aux *.bbl *.blg *.log *.out


